Taming Teacher Forcing for Masked Autoregressive Video Generation

We introduce MAGI, a hybrid video generation framework that combines masked modeling for intra-frame generation with causal modeling for next-frame generation. Our key innovation, Complete Teacher Forcing (CTF), conditions masked frames on complete observation frames rather than masked ones (namely Masked Teacher Forcing, MTF), enabling a smooth transition from token-level (patch-level) to frame-level autoregressive generation. CTF significantly outperforms MTF, achieving a +23% improvement in FVD scores on first-frame conditioned video prediction. To address issues like exposure bias, we employ targeted training strategies, setting a new benchmark in autoregressive video generation. Experiments show that MAGI can generate long, coherent video sequences exceeding 100 frames, even when trained on as few as 16 frames, highlighting its potential for scalable, high-quality video generation.

==> figs/ablation_teacher_forcing.tex <==
\begin{figure}[t!]
    \centering  
    \includegraphics[width=0.45\textwidth]{sec/pic/ablation_tf_mf_2.pdf}
    \caption{\textbf{Masked Teacher Forcing (MTF)} ~\textbf{\textit{v.s.}} \textbf{Complete Teacher Forcing (CTF)}. Both methods utilize the proposed training strategies — dynamic interval training and dynamic noise injection. We report FID scores for individual frames and FVD scores for all frames on UCF101~\cite{soomro2012ucf101}. CTF achieves significantly better FVD scores but slightly worse FID scores compared to MTF. This result demonstrates that MTF better captures motion with temporal coherence, even when the quality of individual frames is lower.}
    \label{fig:ablation_teacher_forcing}
    \vspace{-3mm}
\end{figure}
